Wigner function approach to single electron coherence in quantum Hall edge channels

Recent electron quantum optics experiments performed with on-demand single electron sources call for a mixed time/frequency approach to electronic quantum coherence. Here, we present a Wigner function representation of first order electronic coherence and show that is provides a natural visualization of the excitations emitted by recently demonstrated single electron sources. It also gives a unified perspective on single particle and two particle interferometry experiments. In particular, we introduce a non-classicality criterion for single electron coherence and discuss it in the context of Mach-Zenhder interferometry. Finally, the electronic Hanbury Brown and Twiss and the Hong Ou Mandel experiments are interpreted in terms of overlaps of Wigner function thus connecting them to signal processing.

==> Figures-tex/figure-wigner-lpa-latex.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5102.00,5102.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(900,808){\makebox(0,0){\strut{}-1}}%
      \put(1450,808){\makebox(0,0){\strut{} 0}}%
      \put(2001,808){\makebox(0,0){\strut{} 1}}%
      \put(2551,808){\makebox(0,0){\strut{} 2}}%
      \put(3101,808){\makebox(0,0){\strut{} 3}}%
      \put(3652,808){\makebox(0,0){\strut{} 4}}%
      \put(4202,808){\makebox(0,0){\strut{} 5}}%
      \put(2551,478){\makebox(0,0){\strut{}$\tau/\tau_{\mathrm{e}}$}}%
      \put(728,1094){\makebox(0,0)[r]{\strut{} 0}}%
      \put(728,1721){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(728,2348){\makebox(0,0)[r]{\strut{} 1}}%
      \put(728,2974){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(728,3601){\makebox(0,0)[r]{\strut{} 2}}%
      \put(728,4228){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(134,2661){\rotatebox{-270}{\makebox(0,0){\strut{}$\omega\tau_{\mathrm{e}}$}}}%
    }%
%    \gplgaddtomacro\gplbacktext{%
%    }%
%    \gplgaddtomacro\gplfronttext{%
%      \csname LTb\endcsname%
%      \put(900,808){\makebox(0,0){\strut{}-1}}%
%      \put(1450,808){\makebox(0,0){\strut{} 0}}%
%      \put(2001,808){\makebox(0,0){\strut{} 1}}%
%      \put(2551,808){\makebox(0,0){\strut{} 2}}%
%      \put(3101,808){\makebox(0,0){\strut{} 3}}%
%      \put(3652,808){\makebox(0,0){\strut{} 4}}%
%      \put(4202,808){\makebox(0,0){\strut{} 5}}%
%      \put(2551,478){\makebox(0,0){\strut{}$\tau/\tau_{\mathrm{e}}$}}%
%      \put(728,1094){\makebox(0,0)[r]{\strut{} 0}}%
%      \put(728,1721){\makebox(0,0)[r]{\strut{} 0.5}}%
%      \put(728,2348){\makebox(0,0)[r]{\strut{} 1}}%
%      \put(728,2974){\makebox(0,0)[r]{\strut{} 1.5}}%
%      \put(728,3601){\makebox(0,0)[r]{\strut{} 2}}%
%      \put(728,4228){\makebox(0,0)[r]{\strut{} 2.5}}%
%      \put(134,2661){\rotatebox{-270}{\makebox(0,0){\strut{}$\omega\tau_{\mathrm{e}}$}}}%
%    }%
    \gplbacktext
    \put(0,0){\includegraphics[height=9cm]{Figures-tex/figure-wigner-lpa-latex.png}}%
    \gplfronttext
  \end{picture}%
\endgroup

